Optimal Control of a Free Boundary Problem: Analysis with Second Order Sufficient Conditions

We consider a PDE-constrained optimization problem governed by a free boundary problem. The state system is based on coupling the Laplace equation in the bulk with a Young-Laplace equation on the free boundary to account for surface tension, as proposed by P.\ Saavedra and L.\ R.\ Scott \cite{PSaavedra_RScott_1991}. This amounts to solving a second order system both in the bulk and on the interface. Our analysis hinges on a convex control constraint such that the state constraints are always satisfied. Using only first order regularity we show that the control to state operator is twice continuously Fr\'echet differentiable. We improve slightly the regularity of the state variables and exploit it to show existence of a control together with second order sufficient optimality conditions.

==> 04_Control_to_State/g_diff_preliminaries_2.tex <==
%!TEX root = ../main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Preliminary Estimates (v 2.0)}
\label{sec:G_prelim}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Given that the coupled system \eqref{eq:g_diff_general} is linear, we will use the 
Banach-Ne\v{c}as theorem to prove its well-posedness directly. To this end we shall 
write \ref{eq:g_diff_general} in the more compact form, 
	\begin{align*} \label{eq:g_diff_general_short}
		\BGO\sbr{\gamma, y, \zeta, z} &= F_{\Gamma,\Omega}\del{\zeta, z}
	\end{align*}
where 
	\begin{align*}
		\BGO\sbr{\gamma, y,\zeta,z} &:= \BG\sbr{\gamma,\zeta} + \BO\sbr{y,z+E\zeta;A\sbr{\gop}} 
			+ \BO\sbr{\yop + v,z + E\zeta;\Dif A\sbr\gop\difdir{\gamma}}, \\
		F_{\Gamma,\Omega}\del{\zeta,z} &:= F_\Omega\del{z + E\zeta} + F_\Gamma\del{\zeta}.
	\end{align*}
It then remains to show the both sides of the inf-sup estimates for $\BGO$. 

\begin{lem}[inf-sup side 1]
\end{lem}
\begin{proof} Let $\del{\gamma, y}$ in $\bbW^1$ be fixed but arbitrary. \propref{prop:b_infsup} yields for any $\epsilon > 0$ a pair $\del{\zeta_\gamma, z_y}$ in $\bbV^1:=\sobZ11\Gamma \times \sobZ1q\Omega$ with $\normSZ{\zeta_\gamma}11\Gamma = \normSZ{z_y}1q\Omega = 1$ such that 
	\begin{align*}
		\BG\sbr{\gamma, \zeta_\gamma} + \BO\sbr{y, z_y;A\sbr{\gop}} \geq  \frac1\alpha \normSZ{\gamma}1\infty\Gamma + \frac1\beta \normSZ y 1p\Omega - \epsilon.
	\end{align*}
Furthermore, given $\zeta_\gamma$ above we can obtain a unique $z_\gamma \in \sobZ1q\Omega$ such that for all  $y \in \sobZ 1p\Omega$ we have $\BO\sbr{y, z_\gamma;A\sbr{\gop}} =  -\BO\sbr{y, E\zeta_\gamma;A\sbr{\gop}}$ and 
	\begin{align*}
		\normSZ{z_\gamma}1q\Omega \leq \beta C_A C_E \normSZ{\zeta_\gamma}11\Gamma = \beta C_A C_E.
	\end{align*}
This result being an application of Banach-Ne\v{c}as with the inf-sup estimate \eqref{eq:b2_infsup}.

Next we induce $\bbV^1$ with the equivalent norm $\norm{\del{\zeta, z}}_{\bbV^1} := C_E\normSZ{\zeta}11\Gamma + \normSZ{z}1q\Omega$. Immediately we note that $\norm{\del{\zeta_\gamma, z_y + z_\gamma}}_{\bbV^1} \leq 1 + C_E\del{1+\beta C_A} =: \tilde C$ and thus estimate
	\begin{align*}
		\sup_{0\neq\del{\zeta,z}\in\bbV^1}\frac{\BGO\sbr{\gamma,y,\zeta,z}}{\norm{\del{\zeta,z}}_{\bbV^1}} 
			&\geq \frac{\BGO\sbr{\gamma,y,\zeta_\gamma,z_y+z_\gamma}}{\norm{\del{\zeta_\gamma, z_y+z_\gamma}}_{\bbV^1}} \\
			&\geq \frac{1}{\tilde C}\del{\frac{1}{\alpha}\normSZ{\gamma}1\infty\Gamma + \frac{1}{\beta}\normSZ{y}1p\Omega - \epsilon}	\\
				&\quad -C_A\del{1+\beta C_A}\normSZ{v}1p\Omega\normSZ{\gamma}1\infty\Gamma \\
			&\geq \frac{1}{\tilde C \beta}\norm{\del{\gamma, y}}_{\bbW^1}  - \frac{\epsilon}{\tilde C}
	\end{align*}
provided $\theta_1 \geq 1 - C_E \tilde C\beta C_A / \del{1+\tilde C \beta C_A}.$ The result follows by taking $\epsilon$ to zero.
\end{proof}

\begin{lem}[inf-sup side 2]
\end{lem}
\begin{proof} Let $\del{\zeta, z}$ in $\bbV^1$ be fixed but arbitrary. \propref{prop:b_infsup} yields for any $\epsilon > 0$ a pair $\del{\gamma_\zeta, y_z}$ in $\bbW^1$ with $\normSZ{\gamma_\zeta}1\infty\Gamma = \normSZ{y_z}1p\Omega = 1$ such that 
	\begin{align*}
		\BG\sbr{\gamma_\zeta, \zeta} + \BO\sbr{y_z, z;A\sbr{\gop}} \geq  \frac1\alpha \normSZ{\zeta}1\infty\Gamma + \frac1\beta \normSZ z 1p\Omega - \epsilon.
	\end{align*}
Furthermore, given $y_z$ above we can obtain a unique $\gamma_z \in \sobZ1\infty\Gamma$ such that for all  $\zeta \in \sobZ 11\Gamma$ we have $\BG\sbr{\gamma_z, \zeta} =  -\BO\sbr{y_z, E\zeta;A\sbr{\gop}}$ and 
	\begin{align*}
		\normSZ{\gamma_z}1\infty\Gamma \leq \alpha C_A C_E \normSZ{y_z}1p\Omega = \alpha C_A C_E.
	\end{align*}
This result being an application of Banach-Ne\v{c}as with the inf-sup estimates (\ref{eq:b1_infsup_a}-b).

We can immediately observe that $\normSZ{\gamma_\zeta + \gamma_z}1\infty\Gamma \leq 1+\alpha C_A C_E := \hat C$ and thus estimate
	\begin{align*}
		\BGO\sbr{\gamma_\zeta + \gamma_z,y_z,\zeta,z}
			&\geq \frac1\alpha \normSZ{\zeta}1\infty\Gamma + \frac1\beta \normSZ z 1p\Omega - \epsilon \\
				&\quad - \hat C C_A\del{1+\beta C_A}\normSZ{v}1p\Omega \norm{\del{\zeta, z}}_{\bbV^1} \\
			&\geq \del{\min\del{\frac{1}{\alpha C_E}, \frac 1 \beta} - \hat C\frac{1-\theta_1}{\alpha C_E}}\norm{\del{\zeta, z}}_{\bbV^1}
	\end{align*}

\end{proof}


\begin{prop}[inf-sup condition of $\BGO$]\label{prop:g_prelim} 
\end{prop}
\begin{proof}
For the first part 
\end{proof}

Let $y \in \sobZ{1}{p}{\Omega}$ and consider the operator 
$T:\sobZ1p\Omega \to \sobZ1p\Omega$ given by
	\begin{equation}\label{eq:T_diff_oper}
		T\del{y} := T_2\del{T_1\del{y}} = \yhat
	\end{equation}
where $T_1:\sobZ{1}{p}{\Omega}\to\sobZ{1}{\infty}{\Gamma}$, written as $\ghat := T_1\del{y}$,    
satisfies for every $\zeta \in \sobZ{1}{1}{\Gamma}$
	\begin{align}\label{eq:t1_diff_var}
		\BG\sbr{\ghat,\zeta} + \BO\sbr{\yop+v,E\zeta;\Dif A\sbr\gop\difdir{\ghat}} 
			&= - \BO\sbr{y, E\zeta; A\sbr\gop} \\ 
			&\quad + F_\Omega\del{E\zeta} + F_\Gamma\del\zeta \nonumber
%			&\quad +\pairS{f,E\zeta}p1q\Omega
%			+ \pairS{g,\zeta}{\infty}{1}{1}{\Gamma}, \nonumber
	\end{align}
and $T_2:\sobZ{1}{\infty}{\Gamma}\to \sobZ1p\Omega$, written as $\yhat := T_2\del{\ghat}$,
satisfies for every $z \in \sobZ{1}{q}{\Omega}$
	\begin{align}\label{eq:t2_diff_var}
		\BO\sbr{\yhat, z; A\sbr\gop} 
			= - \BO\sbr{\yop+ v,z;\Dif A\sbr\gop\difdir{\ghat}} 
			+ F_\Omega\del z
			%+ \pairS{f,z}p1q\Omega.
	\end{align}

%%%%%%%
\begin{prop}[inf-sup condition of $T_1$]\label{prop:g_prelim} 
The operator in \eqref{eq:t1_diff_var} satisfies for every $\ghat \in \sobZ1\infty\Gamma$
	\begin{align*}
		\normSZ{\ghat}{1}{\infty}{\Gamma} &\leq \frac{\alpha}{\theta_1} 
			\sup_{0\neq \zeta\in\sobZ{1}{1}{\Gamma}} 
				\frac{\BG\sbr{\ghat,\zeta} + \BO\sbr{\yop+v,E\zeta;\Dif
				A\sbr{\gop}\difdir{\ghat}}}{\normSZ{\zeta}{1}{1}{\Gamma}} .
	\end{align*}
\end{prop}
%%%%%%%
\begin{proof} 
Consider an arbitrary $\zeta \in \sobZ{1}{1}{\Gamma}$ such that $\normSZ{\zeta}{1}{1}{\Gamma} = 1$. 
The $inf$-$sup$ estimate \eqref{eq:b1_infsup_a} together with the continuity of $\BO$ and 
 \eqref{eq:v_invariant} implies
	\begin{align*}
		\sup_{\normSZ{\zeta}{1}{1}{\Gamma}=1} \BG\sbr{\ghat,\zeta} 
			&+ \BO\sbr{\yop + v,E\zeta;\Dif A\sbr\gop\difdir\ghat} \nonumber  \\
		&\geq \frac{1}{\alpha}\normSZ{\ghat}{1}{\infty}{\Gamma} -
			C_EC_A\normSZ{\yop+v}{1}{p}{\Omega} \normSZ{\ghat}{1}{\infty}{\Gamma}  \nonumber \\
		&\geq \del{\frac{1}{\alpha} - C_EC_A\del{1+\beta C_A}\normSZ{v}1p\Omega}\normSZ{\ghat}{1}{\infty}{\Gamma}   \nonumber \\
		&\geq \del{\frac{1}{\alpha} - \frac{{1-\theta_1}}{\alpha}}\normSZ{\ghat}{1}{\infty}{\Gamma}.
	\end{align*} 
The asserted estimate follows immediately.
\end{proof}
%%%%%%%
%%%%%%%
\begin{lem}[well-posedness of $T_1$ and $T_2$] \label{lem:t_diff_maps_back}
Let $T_1$, $T_2$ be the operators in \eqref{eq:t1_diff_var} and \eqref{eq:t2_diff_var} with
$\del{\gop,\yop} \in \bbB_v$. The following holds
\begin{enumerate}[(i)]
	\item\label{item:t_diff_maps_back_b} for every $y \in \sobZ{1}{p}{\Omega}$, there exists an unique $\ghat = T_1\del{y}$ satisfying 
         \eqref{eq:t1_diff_var} and   
         \[
              \normSZ{\ghat}{1}{\infty}{\Gamma} 
              	\leq \frac{\alpha}{\theta_1}\del{
              		\normSZD{F_\Gamma}{1}{1}{\Gamma} + C_E\normSD{F_\Omega}{1}q\Omega
              			+ C_EC_A\normSZ{y}{1}{p}{\Omega}},
         \]
	\item\label{item:t_diff_maps_back_a} for every $\ghat \in \sobZ 1 \infty \Gamma$, there exists an unique $\yhat = T_2(\ghat)$ satisfying 
               \eqref{eq:t2_diff_var} and  
         \[ 
            \normSZ{\yhat}{1}{p}{\Omega} \leq
            	\beta C_A \del{1+\beta C_A}\normSZ{v}1p\Omega\normSZ{\ghat}{1}{\infty}{\Gamma} 
	 				+\beta \normSD{F_\Omega}1q\Omega.
         \]   
\end{enumerate}
\end{lem}
\begin{proof} 
To prove (\ref{item:t_diff_maps_back_b}) we proceed as in \lemref{lem:t_maps_weps} (\ref{item:t_maps_weps_a}).
So it suffices to check that 
%$F\del \zeta := \pairS{g,\zeta}{\infty}{1}{1}{\Gamma} + \pairD{f, E\zeta}{\sob 1 q \Omega} - \BO\sbr{y, E\zeta, A\sbr\gop}$ 
$F\del \zeta := F_\Omega\del{E\zeta} + F_\Gamma\del\zeta - \BO\sbr{y, E\zeta, A\sbr\gop}$ 
is in $\sobZ11\Gamma^*$. This follows directly,
	\begin{align}
		\abs{F\del \zeta} \leq \del{C_E\normSD{F_\Omega}1q\Omega + \normSZD{F_\Gamma}11\Gamma +
			 C_EC_A\normSZ{y}{1}{p}{\Omega}}\normSZ{\zeta}{1}{1}{\Gamma}, 
%		\abs{F\del \zeta} \leq \del{\normLt{g}\Gamma + C_E\normS{f}{-1}p\Omega +
%			 C_EC_A\normS{y}{1}{p}{\Omega}}\normS{\zeta}{1}{1}{\Gamma}, 
	\end{align}
whence $F \in \sobZ{1}{1}{\Gamma}^*$ as required. 
The desired continuity estimate follows from \lemref{lem:baneso} together with $\BG$ being coercive in $\sobZ{1}{2}{\Gamma}$.

Estimate (\ref{item:t_diff_maps_back_a}) is a straightforward application of the Banach-Ne\v{c}as theorem \cite{AErn_JLGuermond_2004a}.
\end{proof}

\begin{thm}[T is a contraction] \label{thm:t_contraction2}  Let $\theta_1 \in \intoo{\beta C_A/(1+\beta C_A), 1}$. Under the assumptions of \lemref{lem:t_diff_maps_back},
$T$ in \eqref{eq:T_diff_oper} is a contraction on $\sobZ{1}{p}{\Omega}$.
\end{thm}
\begin{proof} We proceed in a similar fashion to \thmref{thm:t_contraction}. 
Consider $y_1, y_2 \in \sobZ1p\Omega$ not identical. Using \eqref{eq:T_diff_oper} we have $\ghat_i := T_1\del{y_i}$ and $\yhat_i :=T_2\del{\ghat_i}$ for $i=1,2$. Applying \lemref{lem:t_diff_maps_back} (\ref{item:t_diff_maps_back_b}), together with the lower bound of $\theta_1$, we obtain 
	\begin{align*}
		\normSZ{\ghat_1 - \ghat_2}1\infty\Gamma
			&\leq \frac{\alpha}{\theta_1} C_E C_A\normSZ{y_1 - y_2}{1}{p}{\Omega} \\
			&\leq \frac{1}{\beta C_A}\alpha C_E C_A\del{1+\beta C_A}\normSZ{y_1-y_2}1p\Omega.
	\end{align*}
Similarly,  \lemref{lem:t_diff_maps_back} (\ref{item:t_diff_maps_back_a}) together with \eqref{eq:v_contraction} implies
	\begin{align*}
		\normSZ{\yhat_1 - \yhat_2}{1}{p}{\Omega} 
			&\leq \beta C_A\del{1+\beta C_A}\normSZ{v}1p\Omega\normSZ{\ghat_1 - \ghat_2}{1}{\infty}{\Gamma} \\
			&\leq \alpha C_EC_A\del{1+\beta C_A}^2\normSZ{v}1p\Omega\normSZ{y_1 - y_2}1p\Omega \\
			&\leq \del{1-\theta_2}\normSZ{y_1-y_2}1p\Omega.
	\end{align*}
Hence, $T$ is a contraction as asserted.
\end{proof}
%%%%%%
\begin{cor}[well-posedness of the linear system] \label{cor:g_diff_prelim}
There exists a unique solution $\del{\gamma,y} \in \bbW^1$ to the variational equations \eqref{eq:g_diff_general} and  the following hold
	\begin{subequations}\label{eq:g_diff_prelim_continuity}
	 \begin{align}
		\normSZ{\gamma}{1}{\infty}{\Gamma} 
			&\leq \frac{\alpha}{\theta_1 \theta_2}\del{\normSZD{F_\Gamma}11\Gamma + C_E\del{1+\beta C_A}\normSD{F_\Omega}1q\Omega}, \\
		\normSZ{y}{1}{p}{\Omega} 
		    &\leq \frac{\alpha}{\theta_1 \theta_2}\beta C_A (1+\beta C_A)\normSZ{v}1p\Omega
		    	\del{\normSZD{F_\Gamma}11\Gamma  + C_E \normSD{F_\Omega}1q\Omega} \\
			&\quad+ \frac{\beta}{\theta_2} \normSD{F_\Omega}1q\Omega \nonumber	
	\end{align}
	\end{subequations}
\end{cor}
%%%%%
\begin{proof} 
The existence and uniqueness follows by \thmref{thm:t_contraction2}. We only demonstrate the estimate for $\gamma$ the one for $y$ follows in a similar manner. By applying \lemref{lem:t_diff_maps_back} and the upper bound \eqref{eq:v_contraction} for $v$ we obtain
	\begin{align*}
		\normSZ{\gamma}{1}{\infty}{\Gamma}
			&\leq \frac\alpha{\theta_1}\del{ \normSZD{F_\Gamma}11\Gamma 
				+ C_E\normSD{F_\Omega}1q\Omega
            	+ C_EC_A\normSZ{y}{1}{p}{\Omega}} \\
        	&\leq \frac\alpha{\theta_1}\del{\normSZD{F_\Gamma}11\Gamma  
        		+ C_E\del{1+\beta C_A}\normSD{F_\Omega}1q\Omega} \\
		&\quad + \alpha C_EC_A\del{1+\beta C_A}^2\normSZ{v}1p\Omega\normSZ{\gamma}{1}{\infty}{\Gamma} \\
        	&\leq \frac{\alpha}{\theta_1}\del{\normSZD{F_\Gamma}11\Gamma 
        		+ C_E\del{1+\beta C_A}\normSD{F_\Omega}1q\Omega} + \del{1-\theta_2}\normSZ{\gamma}{1}{\infty}{\Gamma}.
	\end{align*}
Inequality (\ref{eq:g_diff_prelim_continuity}a) follows immediately. 
\end{proof}
%%%%%


==> 04_Control_to_State/g_w2_regularity.tex <==
%!TEX root = ../main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Second order regularity ($\bbW^2$)}
\label{s:g_w2_regularity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Corollary~\ref{cor:g_operator} implies that for every $u\in \Uad$ and $v$ which satisfies 
\eqref{eq:v_invariant} and \eqref{eq:v_contraction} we can find a unique  
solution $(\gamma,y)$ to \eqref{eq:lin_st_const} in $\bbB_v$, i.e. only up to one weak 
derivative for $\gamma$ and $y$.  
In the sequel we will show the solution $\del{\gamma,y} = G_v(u)$ has 
two weak derivatives i.e., $\del{\gamma,y} \in \bbW^2 := \del{\sob{2}{\infty}{\Gamma}\times\sob2p\Omega} \cap \bbW^1$ provided $v \in \sob2p\Omega$ and $u \in \Linf\Gamma$.


%%%%%
\begin{thm}[$\bbW^2$-regularity]  \label{thm:w2_regularity}
Let the assumptions of Corollary~\ref{cor:g_operator} hold with $u\in \Uad \cap \Linf\Gamma$ and with $v$ in $\sob{2}{p}{\Omega}$. Furthermore, let 
	\begin{align*}
		\normS{v}2p\Omega \leq  \\
		\normLi{u}\Gamma \leq 
	\end{align*}
then \eqref{eq:lin_st_const} has a unique solution $\del{\gamma, y}$ with $\bbW^2$-regularity.
\end{thm}
%%%%%
\begin{proof} 
The proof is the the contraction in \thmref{thm:t_contraction} under the more restrictive set  
\[
   \bbB^2_v := \set{(\gamma,y) \in \bbW^2 :\;
		\norm{y}_\sob{2}{p}{\Omega} \leq \beta C_A \normS v 2 p \Omega,\; \normS{\gamma}2\infty\Gamma \leq 1},
\]   
Solving the boundary value problem  $\gtl = T_1(\gamma,y)$ yields 
	\begin{align*}
		\normSZ{\gamma}2\infty\Gamma 
			\leq \frac{1}{\kappa}C_A C_{\cembed{\sob2p\Omega}{\sob1\infty\Omega}} \normS{y}2p\Omega + \normLi{u}\Gamma
	\end{align*}
%	\begin{align*}
%		\gtl(x_1) 
%			&= -\frac 1 \kappa \int_0^{x_1}\int_0^\tau A\sbr{\gamma_0}\ngrad\del{y+v}- u(\tau_1)\dif \tau_1\dif \tau \\
%			&\quad+ x_1\frac 1 \kappa \int_0^1\int_0^\tau A\sbr{\gamma }\ngrad\del{y+v}- u(\tau_1)\dif \tau_1\dif \tau.
%	\end{align*}	
In other words, $\gtl \in \sob2\infty\Gamma\cap\sobZ1\infty\Gamma$, since $u$ and $A\sbr{\gamma}\grad\del{y+v} \cdot \nu$ are both 
in $\Linf\Gamma$, the former because of the box-constraints and latter because by Sobolev embedding theorem. We now turn to the solution of the PDE,  $\ytl = T_2(\gtl, \cdot)$, which in non-divergence form reads
	\begin{align*}
		-A\sbr{\gamma}\lapl (\ytl + v)  - \grad{A\sbr{\gamma}}\cdot\grad\del{\ytl + v} &= 0 && \env{in } \Omega
	\end{align*}
with $\ytl = 0$ on $\bdy\Omega$. Due to the structure of $A$, it follows that $A\sbr{\gtl}$ is Lipschitz. Therefore, we apply  \cite[Theorem 9.15]{DGilbarg_NTrudinger_2001a} to infer the higher regularity $\ytl \in \sob2p\Omega\cap\sobZ1p\Omega$.  
Then a similar contraction argument to Theorem~\ref{thm:t_contraction} leads to the claim of assertion. 

\end{proof}

==> g_uu_lipschitz.tex <==
%!TEX root = main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{$G_v''$ is Lipschitz}
\label{s:g_uu_lipschitz}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this last subsection we will show that $G_v''$ is Lipschitz. 
%%%%
\begin{thm}[$G_v''$: Lipschitz Continuity]  \label{thm:g_uu_lipschitz} 
Let $v \in \Vad$ be given then $G_v''$ is Lipschitz continuous with respect to $u \in \Uad$, 
with a Lipschitz constant $L_{G2} > 0$, i.e., given $u_1, u_2 \in \Uad$, $u_1 \neq u_2$ and $h \in
\cone{u_1} \cap \cone{u_2}$ we have
\begin{align} \label{eq:g_uu_lipschitz}
   \norm{G_v''(u_1)h^2 - G_v''(u_2)h^2}_\Weps \leq L_{G2}\norm{u_1-u_2}_\Uad.
\end{align}   
\end{thm}
%%%%
\begin{proof} 
Set $G_v(u_1) - G_v(u_2) := \del{\gamma_1,y_1} - \del{\gamma_2, y_2}$, then using 
\eqref{eq:g_var_pde}, we have for every $r \in \sobZ{1}{q}{\Omega}$ and $s \in \sobZ 1 1 \Gamma$
	\begin{equation*}\label{eq:g_difference}\left\{\begin{aligned}
		B_2\sbr{y_1+v,r;A\sbr{\gamma_1}} - B_2\sbr{y_2+v,r;A\sbr{\gamma_2}}&= 0 	 \\ 
	    B_1\sbr{\gamma_1-\gamma_2,s} + B_2\sbr{y_1+v,Es;A\sbr{\gamma_1}} 
	    	- B_2\sbr{y_2+v,Es;A\sbr{\gamma_2}} &= \pair{u_1 - u_2,s}
	\end{aligned}\right..\end{equation*}
	By adding and subtracting $B_2\sbr{y_2,\cdot;A\sbr{\gamma_1}}$ to the first and second equations 
	and rearranging terms we obtain 			
	\begin{equation*}\left\{\begin{aligned}
		B_2\sbr{y_1-y_2,r;A\sbr{\gamma_1}} &= B_2\sbr{y_2+v,r;A\sbr{\gamma_2}-A\sbr{\gamma_1}} \\ 
	    B_1\sbr{\gamma_1-\gamma_2,s} &= B_2\sbr{y_2-y_1,Es;A\sbr{\gamma_1}} \\ 
	    	&\quad + B_2\sbr{y_2+v,Es;A\sbr{\gamma_2}-A\sbr{\gamma_1}} + \pair{u_1 - u_2,s}	 
	\end{aligned}\right..\end{equation*}
	The $\inf$-$\sup$ estimates from \propref{prop:b_infsup} and $\delta_v$ from 
	(\ref{eq:e_v_u_est}b) implies
	\begin{align*}
		\normS{y_1-y_2}{1}{p}{\Omega} 
			&\leq \beta C_A\normS{y_2+v}{1}{p}{\Omega} \normS{\gamma_1-\gamma_2}{1}{\infty}{\Gamma} \\ 
			&\leq \del{1+\beta C_A }\epsilon\norm{\gamma_1-\gamma_2}_\sob{1}{\infty}{\Gamma} , \\
		\normS{\gamma_1 - \gamma_2}{1}{\infty}{\Gamma}
			&\leq \alpha C_EC_A\del{\normS{y_1-y_2}{1}{p}{\Omega}
				+ \normS{y_2+v}{1}{p}{\Omega}\normS{\gamma_1 - \gamma_2}{1}{\infty}{\Gamma}} \\
			&\quad + \alpha \norm{u_1 - u_2}_\Uad \\ 
			&\leq \frac{\alpha}{\beta}C_E\del{1 + \beta C_A }^2
				\epsilon\normS{\gamma_1-\gamma_2}{1}{\infty}{\Gamma}
				+\alpha \norm{u_1-u_2}_\Uad \\
			&\leq \frac{4}{3}\alpha \norm{u_1-u_2}_\Uad .\hspace*{4cm} \env{using (\ref{eq:e_v_u_est}a)}
	\end{align*}
    Therefore \eqref{eq:g_lipschitz} follows with $L_G = \frac{4}{3}\alpha\epsilon\del{2+\beta C_A}$.
\end{proof}
%%%%

==> leftovers.tex <==
%!TEX root = main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% 2nd Order Conditions identies, relations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Relations to be exploited by multiplying \eqref{eq:lin_prob} by the optimal adjoint states $r$ and $s$
\begin{enumerate}
	\item $B_1\sbr{y, r; A\sbr{\bar\gamma}} = -B_1\sbr{\bar y, r; \Dif A\sbr{\bar\gamma}\gamma} - \int_\Gamma s\del{\nd_{A}y + \nd_{\Dif A\gamma} \bar y}$. Furthermore, since $r$ is optimal and $y = 0$ on the boundary, we obtain the identity 
		\begin{equation}B_1\sbr{\bar y, r; \Dif A\sbr{\bar\gamma}\gamma} = -\lambda_y \int_\Omega y\del{\bar y - y_d} -\int_\Gamma s\del{\nd_{A}y + \nd_{\Dif A\gamma}\bar y}.\end{equation}
	\item $B_2\sbr{\gamma, s} = \int_\Gamma s\del{\nd_{A}y + \nd_{\Dif A\gamma}\bar y} + \int_\Gamma su$, which when put together with the previous item gives us 
		\begin{equation}B_1\sbr{\bar y, r;\Dif A\sbr{\bar\gamma}\gamma} = -\lambda_y \int_\Omega y\del{\bar y - y_d} -B_2\sbr{\gamma, s} + \int_\Gamma su.\end{equation}
	\item We exploit that $s$ is optimal to obtain this new identity 
		\begin{equation}
			0 = -\lambda_y \int_\Omega y\del{\bar y - y_d} -\lambda_\gamma\int_\Gamma \gamma\del{\bar \gamma - \gamma_d} + \int_\Gamma su.
		\end{equation}
	\item We exploit the pairing $\bar \gamma$ with $s$ with the residual of $\bar y$ paired with $r$ to get
		\begin{subequations}\begin{align}
			B_1\sbr{\bar y, r;A\sbr{\bar \gamma}} &= \int_\Gamma r \nd_A \bar y = -\int_\Gamma s\nd_A \bar y \\
			B_2\sbr{\bar \gamma, s} &= \int_\Gamma s\nd_A \bar y + \int_\Gamma s\bar u \\
			B_1\sbr{\bar y, r;A\sbr{\bar \gamma}} + B_2\sbr{\bar \gamma, s} &= \int_\Gamma s\bar u \\
			B_1\sbr{\bar y, r;A\sbr{\bar \gamma}} &= \lambda_y\int_\Omega \bar y\del{\bar y -y_d} + \int_{\bdy\Omega}g\nd_A r  \\
			B_2\sbr{\bar \gamma, s} &= \lambda_\gamma \int_\Gamma \bar \gamma\del{\bar \gamma - \gamma_d} - B_1\sbr{\bar y, r;\Dif A\sbr{\bar \gamma}\bar \gamma}
		\end{align}\end{subequations}
	\item Combine previous two items to get
		\begin{align}
			B_1\sbr{\bar y, r; \Dif A\sbr{\bar \gamma}\bar \gamma} - \int_{\bdy\Gamma}g \nd_A r &= 
				\lambda_y \pair{\bar y - y, \bar y - y_d} + \lambda_\gamma \pair{\bar \gamma - \gamma, \bar \gamma - \gamma_d} + \int s\del{u - \bar u}
		\end{align}
	\item We need to continuing using the equations to finish our proof, you want to have everything in terms of the differences $\bar y - y$, $\bar\gamma - \gamma$, $\bar u - u$.
\end{enumerate}

\begin{align}
	\lagr''\del{\bar{ }}\difdir{y,\gamma,u}^2 
		&= \lambda_y\normLt{y}{\Omega}^2 + \lambda_\gamma\normLt{\gamma}{0,1}^2 + \lambda_u\normLt{u}{0,1}^2 \\
		 &\quad -B_1\sbr{\bar y, r;\Dif^2 A\sbr{\bar\gamma}\gamma^2} -B_1\sbr{y, r;\Dif A\sbr{\bar \gamma}\gamma} \\
		&=	... -B_1\sbr{\bar y, r;\Dif^2 A\sbr{\bar\gamma}\gamma^2} 
		    +\underbrace{B_1\sbr{\bar y-y, r;\Dif A\sbr{\bar\gamma}\gamma}}_{\geq -C\norm{\bar y - y}} - B_1\sbr{\bar y, r;\Dif A\sbr{\bar\gamma}\gamma} \\
		&= ... -B_1\sbr{\bar y, r;\Dif^2 A\sbr{\bar\gamma}\gamma^2} + B_2\sbr{\gamma, s} + \lambda_y\pair{y, \bar y - y_d}  -\int_\Gamma su \\
		&= ... -B_1\sbr{\bar y, r;\Dif^2 A\sbr{\bar\gamma}\gamma^2} + \underbrace{B_2\sbr{\gamma - \bar\gamma,s}}_{\geq - C\norm{\bar \gamma - \gamma}} + B_2\sbr{\bar\gamma,s} - \int_\Gamma su \\
		&= ... -B_1\sbr{\bar y, r;\Dif^2 A\sbr{\bar\gamma}\gamma^2} + \int_\Gamma s\nd_A \bar y + \underbrace{\int_\Gamma s\del{\bar u - u}}_{\geq -C\norm{\bar u - u}} \\ 
		&= ... -B_1\sbr{\bar y, r;\Dif^2 A\sbr{\bar\gamma}\gamma^2} - \int_{\bdy\Gamma} r\nd_A \bar y \\
		&= ... -B_1\sbr{\bar y, r;\Dif^2 A\sbr{\bar\gamma}\gamma^2} - B_1\sbr{\bar y, r; A\sbr{\bar \gamma}} \\
		&= ... -B_1\sbr{\bar y, r; A\sbr{\bar \gamma} + \Dif^2 A\sbr{\bar\gamma}\gamma^2}
\end{align}

==> regularity.tex <==
%!TEX root = main.tex

\section{Well-Posedness and Regularity of State Constraints}
In this section we want to find conditions on fixed $u$ and $g$ to guarantee the existence and uniqueness of a solution to the the state constraints equation \eqref{eq:state_constraint}. The proof is a fixed-point argument. First we introduce some function space

\begin{defn} Let $B_\epsilon := \setdef{\del{\gamma,y} \in Z\times Y}{\sobGammaSNorm{\gamma} < 1,\; \sobOmegaNorm{y} < \epsilon}$, where $Z:=\sobTGamma\cap\sobZGamma$ and $Y:=\sobTOmega\cap\del{g\oplus\sobZOmega}$ with $p>2$.We will later show that $B_\epsilon$ is our invariant space.
\end{defn}

\begin{defn} Let $T_1$ be the map taking $\del{\gamma_0, y_0} \in B_\epsilon$ into $\gamma \in Z$ where $\gamma$ is the solution to the boundary value problem, 
	\begin{align}\label{eq:lin_mean_curv}
		-\kappa \dod{}{x}\del{\frac{\dot\gamma(x)}{\sqrt{1+{\dot{\gamma_0}(x)^2}}}} &= \nd y(x, 1+\gamma_0(x)) + u(x)   && x \in \intoo{0,1}
	\end{align} 
\end{defn}

\begin{prop} Let $\gamma$ be in the range of $T_1$ and $u \in \Linf{0,1}$, then \eqref{eq:lin_mean_curv} admits a closed form solution in $Z$ given by $$\gamma(x) = \int_0^x A^{-1}\del{t;\gamma_0}\del{C_1 - \int_0^t f(s;\gamma_0,y,u) \dif s}\dif t$$
where $A(x;\gamma_0):= \kappa/\sqrt{1 + \dot{\gamma_0}(x)^2}$, $f(x;\gamma_0,y,u) := \nd y(x,1+\gamma_0(x)) + u(x)$ and $C_1 = \del{\int_0^1\int_0^t f(s)/A(t)\dif s\dif t}/\del{\int_0^1 1/A(t) \dif t}$. Furthermore, ....

\begin{proof} First, verification of the closed form solution is a calculus exercise which we skip. Second, for $y \in Y$ with $p > 2$ we obtain by Sobolev embedding that $\trace{\grad y} \in \sob{1-1/p}{p}{\bdy\Omegag} \subset \Linf{\bdy\Omegag}$ and therefore since $\gamma_0$ is Lipschitz, $\nd y(x,1+\gamma_0(x)) \in \Linf{0,1}$ with $\norm{\nd y}_{\Linf{0,1}} \leq C \sobOmegaNorm{y}$ where $C$ does not depend on $y_0$. Together with the assumption that $u \in \Linf{0,1}$ we obtain that $f(\cdot;\gamma_0,y,u) \in \Linf{0,1}$ as well. Third, since $\sobGammaSNorm{\gamma_0} \leq 1$, we obtain that $$\frac{\kappa}{\sqrt{2}} \leq A(x;\gamma_0) \leq \kappa \quad \aev x \intoo{0,1}.$$ Fourth, $\abs{C_1}$ is upper bounded by $\sqrt{2}\norm{f}_{\Linf{0,1}}$. Finally, we obtain the estimate 
\begin{align*}
	\sobGammaSNorm{\gamma} &:= \esssup \abs{\dot{\gamma}(x)}  \\
		&= \leq \norm{A^{-1}}_{\Linf{0,1}}\del{\abs{C_1} + \norm{f}_{\Linf{0,1}}} \\
		&\leq C\del{\sobOmegaNorm{y} + \norm{u}_{\Linf{0,1}}} \\
		&\leq C\del{\epsilon + \norm{u}_{\Linf{0,1}}} \\
		&\leq 1
\end{align*}
provided $\epsilon$ is small enough and $\norm{u}_{\Linf{0,1}} \leq 1/c - \epsilon$.
\end{proof}
\end{prop}

\begin{defn} Let $T_2$ be the map taking $\del{\gamma_0, y_0} \in B_\epsilon$ into $y \in Y$ where $y$ solves the PDE, 
	\begin{align}\label{eq:harm_omegag}
		-\lapl y &= 0 && \env{in } \Omega_{\gamma_0}
	\end{align}
\end{defn}

\begin{prop} Let $y$ be in the range of $T_2$, then for $g$ suitably small, $y \in Y$.
\begin{proof} Flatten the boundary. Notice the matrix $A(x;\gamma_0)$ in Saavedra and Scott is now Lipschitz continuous. Apply Theorem 9.15 in \cite[GiTr89] to conclude $y \in \sobTOmega$ and $\norm{y}_{\sobTOmega} \leq C\norm{g}$
\end{proof}
\end{prop}

